Iterative Geometry Calibration from Distance Estimates for Wireless Acoustic Sensor Networks

In this paper we present an approach to geometry calibration in wireless acoustic sensor networks, whose nodes are assumed to be equipped with a compact microphone array. The proposed approach solely works with estimates of the distances between acoustic sources and the nodes that record these sources. It consists of an iterative weighted least squares localization procedure, which is initialized by multidimensional scaling. Alongside the sensor node locations, also the positions of the acoustic sources are estimated. Furthermore, we derive the Cramer-Rao lower bound (CRLB) for source and sensor position estimation, and show by simulation that the estimator is efficient.

==> commands.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = Schmalen2020.tex
% !TeX program = pdflatex
% !BIB program = bibtex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\zB}{z.~B.\xspace}
\newcommand{\dhAbbrev}{d.~h.\xspace}
\newcommand{\vgl}{vgl.\xspace}
\newcommand{\sog}{sog.\xspace}
\newcommand{\ua}{u.~a.\xspace}
\newcommand{\bspw}{bspw.\xspace}
\newcommand{\bzw}{bzw.\xspace}
\newcommand{\ca}{ca.\xspace}
\newcommand{\ggf}{ggf.\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% basic math style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\grad}{\ensuremath{^\circ}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\scr}[1]{\ensuremath{\mathcal{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mathematical operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\sinc}{sinc}
\renewcommand{\Re}{Re}
\renewcommand{\Im}{Im}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\ee}{\mathrm e}
\newcommand{\jj}{\mathrm j}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rect}{\ensuremath{{\rm rect}}}
\newcommand{\sgn}{\ensuremath{{\rm sgn}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% fourier-transformation, z-transformation 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\FT}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\text{---}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IFT}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\text{---}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}
\newcommand{\ZT}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\overset{z}{\text{---}}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IZT}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\overset{z^{-1}}{\text{---}}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}
\newcommand{\ZTE}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\overset{z_1}{\text{---}}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IZTE}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\overset{z_1^{-1}}{\text{---}}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% other
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\SNR}{\ensuremath{{\rm SNR}}}
\newcommand{\SINR}{\ensuremath{{\rm SINR}}}
\newcommand{\Prob}{\ensuremath{{\rm Prob}}}
\newcommand{\rb}[1]{\raisebox{1.5ex}[-1.5ex]{#1}}
\newcommand{\erf}{\ensuremath{{\rm erf}}}
\newcommand{\erfc}{\ensuremath{{\rm erfc}}}



%\newacronym{PESQ}{PESQ}{Perceptual Evaluation of Speech Quality}
%\newacronym{ATF}{ATF}{Acoustic Transfer Function}
%\newacronym{STFT}{STFT}{Short Time Fourier Transform}
%\newacronym{FFT}{FFT}{Fast Fourier Transform}
%\newacronym{IFFT}{IFFT}{Inverse Fast Fourier Transform}
%\newacronym{MVDR}{MVDR}{Minimum Variance Distortionless Response}
%\newacronym{DSB}{DSB}{Delay-and-Sum Beamformer}
%\newacronym{TDOA}{TDOA}{Time Differences of Arrival}
%\newacronym{GEV}{GEV}{Generalized Eigenvalue}
%\newacronym{BAN}{BAN}{Blind Analytic Normalization}
%\newacronym{BLSTM}{BLSTM}{bi-directional Long Short-Term Memory}
%\newacronym{ReLU}{ReLU}{Rectified Linear Unit}
%\newacronym{FF}{FF}{feed-forward}
%\newacronym{SNR}{SNR}{signal-to-noise ratio}
%
%\newacronym{SINR}{SINR}{Signal-to-Interference-Noise Ratio}

%\newacronym{SDR}{SDR}{signal-to-distortion ratio}
%\newacronym{DNN}{DNN}{Deep Neural Network}
%\newacronym{ASR}{ASR}{Automatic Speech Recognition}
%\newacronym{DOA}{DoA}{Direction-of-Arrival}
%\newacronym{CDR}{CDR}{Coherence-to-Diffuse-Ratio}
%\newacronym{GMM}{GMM}{Gaussian Mixture Model}
%\newacronym{WER}{WER}{word error rate}
%\newacronym{PSD}{PSD}{Power Spectral Density}
%\newacronym{CNN}{CNN}{Convolutional Neural Network}
%\newacronym{EM}{EM}{Expectation-Maximization}
%\newacronym{tf}{tf}{time frequency}
%\newacronym{gcc}{GCC}{generalized cross correlation}
%\newacronym{CE}{CE}{Cross-Entropy}
%\newacronym{WRN}{WRN}{Wide Residual Network}
%\newacronym{SRO}{SRO}{Sampling Rate Offset}
%\newacronym{ACD}{ACD}{Average Coherence Drift}
%\newacronym{WACD}{WACD}{Weighted Average Coherence Drift}
%\newacronym{WASN}{WASN}{Wireless Acoustic Sensor Networks}
%\newacronym{ADC}{ADC}{Analog-to-Digital Converter}
%\newacronym{VAD}{VAD}{Voice Activity Detection}
%\newacronym{RMSE}{RMSE}{Root Mean Square Error}
%\newacronym{OSM}{OSM}{Overlap-Save method}
%\newacronym{GaBP}{GaBP}{Gaussian Belief Propagation}
%\newacronym{WLAN}{WLAN}{Wireless Local Area Network}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Source code listings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings}
\usepackage{textcomp}
% define MATLAB highlighting
\lstdefinelanguage{matlabNT}{ alsoletter={...}, %
                              morekeywords={ % keywords
                              break,case,catch,continue,elseif,else,end,for,
                              function,global,if,otherwise,persistent,return,
                              switch,try,while,...},
                              comment=[l]\%,% the comment sign comments
                              morecomment=[l]..., % if a command is split over multiple lines
                              morestring=[m]', %strings
}[keywords,comments,strings]

% define the wanted font for all highlightings here
\def\lstbasicfont{\fontfamily{pcr}\selectfont}
\lstset{  language=matlabNT,                            % use our version of highlighting
          keywordstyle=\color[rgb]{0,0,1},              % keywords
          commentstyle=\color[rgb]{0.133,0.545,0.133},  % comments
          stringstyle=\color[rgb]{0.627,0.126,0.941},   % strings
          captionpos=b,                                 % the caption position --> b:bottom
          basicstyle={\lstbasicfont
                      \footnotesize
                      \color[rgb]{0,0,0}},              % use defined font, smaller size and default textcolor black
          showstringspaces=false,                       % do not emphasize spaces in strings
          tabsize=2,                                    % number of spaces of a TAB
          mathescape=true,escapechar=§,                 % escape to latex with §...§
          upquote=true,                                 % upright quotes
          aboveskip={1.5\baselineskip},                 % a bit of space above
          columns=fixed,                                % nice spacing
          %backgroundcolor=\color[rgb]{0.95,0.95,0.95},  % the background color will be light gray
          numbersep=3mm,                                % spacing between numbers and text/code
          numbers=left,                                 % numbers are left
          numberstyle=\tiny,                            % numbers are tiny
          frame=trbl,                                   % single frame at top, right, bottom and left, capital letters
                                                        % produce double-lined frames
          frameround=tttt,                              % round corners
          framexleftmargin=6mm,                         % tweak margins
          xleftmargin=6mm,                              % tweak margins
          % the following is for replacing some matlab relations like >= or ~=
          % by the corresponding LaTeX symbols, which are much easier to read ...
          literate=%
            {~}{{$\neg$}}1            % \neg
            {<=}{{\tiny$\leq$}}1      % \leq
            {>=}{{\tiny$\geq$}}1      % \geq
            {~=}{{\tiny$\neq$}}1      % \neq
            {delta}{{\tiny$\Delta$}}1 % \Delta
}


==> sections/dnn.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = Schmalen20ITG.tex
% !TeX program = pdflatex
% !BIB program = bibtex


\section{DNN based distance estimation} \label{SEC:DNN}
Brendel et.al, introduced in \cite{brendel_distributed_2019} and \cite{brendel_probabilistic_2019} a \gls{CDR}-based distance estimation. It utilized \gls{GP} regression trained on the averaged diffuseness for distance estimation. However, the need to learn an environment prohibited the application to unknown rooms and therefore the application in geometry calibration tasks.
Furthermore, the inherent distance dependence of the variance of the distance estimates as reported in \cite{brendel_distributed_2019, Gburrek2020} is crucial to geometry calibration tasks. Even a few outliers with extraordinary distance estimation errors can effectively dominate the geometry layout, if the approach tries to minimize a quadratic cost function and therefore focuses on the outliers.

In \cite{Gburrek2020} we presented a \gls{DNN} based distance estimator for supporting geometry calibration tasks in \glspl{WASN}. It overcomes the restriction of the \gls{GP} based approach by incorporating training data of multiple environments into the \gls{DNN} training process, enabling generalization to unseen acoustic environments. Additionally, the \gls{DNN} assigns observations to a \gls{OoR} called class if the distance probably results in unreliable estimates. In the following, the \gls{DNN} distance estimator from \cite{Gburrek2020} is employed for all experiments. 
